Iterative Token Evaluation and Refinement for Real-World Super-Resolution

Real-world image super-resolution (RWSR) is a long-standing problem as low-quality (LQ) images often have complex and unidentified degradations. Existing methods such as Generative Adversarial Networks (GANs) or continuous diffusion models present their own issues including GANs being difficult to train while continuous diffusion models requiring numerous inference steps. In this paper, we propose an Iterative Token Evaluation and Refinement (ITER) framework for RWSR, which utilizes a discrete diffusion model operating in the discrete token representation space, i.e., indexes of features extracted from a VQGAN codebook pre-trained with high-quality (HQ) images. We show that ITER is easier to train than GANs and more efficient than continuous diffusion models. Specifically, we divide RWSR into two sub-tasks, i.e., distortion removal and texture generation. Distortion removal involves simple HQ token prediction with LQ images, while texture generation uses a discrete diffusion model to iteratively refine the distortion removal output with a token refinement network. In particular, we propose to include a token evaluation network in the discrete diffusion process. It learns to evaluate which tokens are good restorations and helps to improve the iterative refinement results. Moreover, the evaluation network can first check status of the distortion removal output and then adaptively select total refinement steps needed, thereby maintaining a good balance between distortion removal and texture generation. Extensive experimental results show that ITER is easy to train and performs well within just 8 iterative steps. Our codes will be available publicly.

==> tab_synthetic.tex <==
\begin{table*}[t]
    \caption{Quantitative comparison with state-of-the-art methods on synthetic benchmarks. LR images are generated with a mixed degradation model of BSRGAN \cite{zhang2021designing} and Real-ESRGAN \cite{wang2021real}. PSNR/SSIM $\uparrow$: the higher, the better; LPIPS $\downarrow$: the lower, the better. LPIPS scores can better reflect texture quality, and the best and second performance are marked in \red{red} and \textcolor{blue}{blue}.} \label{tab:synthetic}
    \setlength{\tabcolsep}{1pt}
    \renewcommand*{\arraystretch}{1.2}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{|c|c|cc|c|cc|c|cc|c|cc|c|cc|c|cc|c|}
    \hline
    \multirow{2}{*}{Method} & \multirow{2}{*}{Scale} & \multicolumn{3}{c|}{DIV2K Valid} & \multicolumn{3}{c|}{Set5} & \multicolumn{3}{c|}{Set14} & \multicolumn{3}{c|}{BSD100} & \multicolumn{3}{c|}{Urban100} & \multicolumn{3}{c|}{Manga109} \\ \cline{3-20} 
     &  & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS \\ \hline
    BSRGAN & $\times2$ & 26.60 & 0.7073 & 0.3182 & 27.65 & 0.7799 & 0.2027 & 24.59 & 0.6475 & 0.3013 & 24.88 & 0.5967 & 0.3769 & 22.76 & 0.6391 & 0.3199 & 24.64 & 0.7678 & 0.2285 \\ 
    Real-ESRGAN+ & $\times2$ & 25.50 & 0.6963 & 0.2993 & 26.73 & 0.7771 & 0.2157 & 23.65 & 0.6299 & 0.3023 & 24.11 & 0.5860 & 0.3433 & 21.66 & 0.6148 & 0.2876 & 23.88 & 0.7698 & 0.2135 \\  
    SwinIR-GAN & $\times2$ & 25.33 & 0.6886 & 0.3313 & 27.07 & 0.7793 & 0.2093 & 23.76 & 0.6364 & 0.3128 & 23.83 & 0.5717 & 0.3707 & 21.54 & 0.6195 & 0.3003 & 23.56 & 0.7705 & 0.2283 \\ 
    FeMaSR & $\times2$ & 25.26 & 0.6680 & 0.2753 & 26.46 & 0.7470 & 0.1964 & 23.38 & 0.5982 & 0.2852 & 23.83 & 0.5599 & 0.3264 & 21.90 & 0.5956 & 0.2777 & 23.64 & 0.7407 & 0.2192 \\ 
    \textbf{Ours} & $\times2$ & 
    \\ \hline \hline
    BSRGAN & $\times4$ & 24.91 & 0.6500 & 0.3596 & 21.63 & 0.5573 & 0.4683 & 22.17 & 0.5165 & 0.4173 & 22.95 & 0.5042 & 0.4405 & 20.91 & 0.5386 & 0.3874 & 22.45 & 0.6968 & 0.3039 \\ 
    Real-ESRGAN+ & $\times4$ & 23.80 & 0.6414 & 0.3696 & 21.31 & 0.5449 & 0.5068 & 21.54 & 0.5288 & 0.4271 & 22.43 & 0.5035 & 0.4693 & 19.90 & 0.5282 & 0.3838 & 21.97 & 0.6989 & 0.3073 \\ 
    SwinIR-GAN & $\times4$ & 24.13 & 0.6479 & 0.3543 & 20.91  & 0.5128 & 0.5115 & 21.58 & 0.5041 & 0.4487 & 22.23 & 0.4925 & 0.4447 & 20.01 & 0.5300 & 0.3592 & 22.21 & 0.7007 & 0.3044 \\ 
    FeMaSR & $\times4$ & 23.77 & 0.6203 & 0.3298 & 20.45 & 0.4863 & 0.4942 & 21.24 & 0.4809 & 0.3801 & 22.11 & 0.4830 & 0.4143 & 20.25 & 0.5243 & 0.3566 & 21.98 & 0.6816 & 0.2846 \\ 
    LDM-BSR & $\times4$ &  \\ \hline
    \textbf{Ours} & $\times4$ &  \\ \hline
    \end{tabular}
    }
\end{table*}
